Mirror Descent on Reproducing Kernel Banach Spaces

Recent advances in machine learning have led to increased interest in reproducing kernel Banach spaces (RKBS) as a more general framework that extends beyond reproducing kernel Hilbert spaces (RKHS). These works have resulted in the formulation of representer theorems under several regularized learning schemes. However, little is known about an optimization method that encompasses these results in this setting. This paper addresses a learning problem on Banach spaces endowed with a reproducing kernel, focusing on efficient optimization within RKBS. To tackle this challenge, we propose an algorithm based on mirror descent (MDA). Our approach involves an iterative method that employs gradient steps in the dual space of the Banach space using the reproducing kernel. We analyze the convergence properties of our algorithm under various assumptions and establish two types of results: first, we identify conditions under which a linear convergence rate is achievable, akin to optimization in the Euclidean setting, and provide a proof of the linear rate; second, we demonstrate a standard convergence rate in a constrained setting. Moreover, to instantiate this algorithm in practice, we introduce a novel family of RKBSs with $p$-norm ($p \neq 2$), characterized by both an explicit dual map and a kernel.

==> sections/conclude.tex <==
\section{Conclusion} \label{sec: conclude}



==> sections/mirror_map.tex <==
\subsection{Mirror Maps}\label{subsec: mirrormap}
Consider a convex open set of functionals $\cC$ such that $\cB \subset \Bar{\cC}$. We are interested in certain real-valued functionals on $\cC$ for the mirror descent algorithm of \eqnref{eq: MD} that could be used to map functions in the primal space $\cB$ to transformations in $\cB^*$. 

In \secref{subsec: probsetup} we introduced mirror maps to discuss the mirror descent algorithms in \eqnref{eq: prelmd}. Formally, we define mirror maps as follows:

\begin{definition}[Mirror Map]\label{def: mp} We say that a functional $\Phi: \cC \to \reals$ is a mirror map if it satisfies the following properties:
\begin{enumerate}[leftmargin=3em]
    \item $\Phi$ is strictly convex and differentiable.
    \item $\partial_{(\cdot)}\Phi$ is one-to-one and onto, i.e. $\partial_{(\cdot)} \Phi (\cB) = \cB^*$.
    \item $\Phi$ diverges on the boundary of $\cC$, i.e. $\lim_{f \to \partial \cC} \norm{\partial_f \Phi}_{\cB^*} = + \infty.$
\end{enumerate}
\end{definition}

%\paragraph{Mirror map} We consider a strictly convex differentiable map $\Phi: \cB \to \reals$ termed as \tt{mirror map} to project any function $f \in \cB$ to the dual space $\cB^*$. Note that at any point $h \in \cB$, the Frech$\acute{e}$t derivative of $\Phi$ satisfies the following:
%\begin{align*}
%    h \mapsto \partial_h \Phi \in \cB^*
%\end{align*}
%In this section, we consider a mirror map defined on a convex open set of functions $\cC$ such that $\cB \subset \Bar{\cC}$ and in addition satisfies the following properties:
%\begin{enumerate}[leftmargin=3em]
%    \item $\Phi$ is strictly convex and differentiable.
%    \item $\partial_{(\cdot)}\Phi$ is one-to-one and onto, i.e. $\partial_{(\cdot)} \Phi (\cB) = \cB^*$.
%    \item $\Phi$ diverges on the boundary of $\cC$, i.e. $$\lim_{f \to \partial \cC} \norm{\partial_f \Phi}_{\cB^*} = + \infty.$$
%\end{enumerate}

The property \tt{2.} above is the key ingredient to the MDA in \eqnref{eq: MD}. The injectivity makes sure that the algorithm could converge without getting stuck in a loop and the surjectivity makes sure that the algorithm gets back to the primal space reliably.
The algorithm would make sense only if the chosen mirror map satisfies this property. We can guarantee this  for any strictly convex and G\^{a}teaux differentiable functional $\msf F: \cB \to \reals$. We would rather prove a strong result in \lemref{lemma: inversemirror} to establish that. First, we state a useful lemma on the first-order optimality condition for optimization in functional analysis.
\begin{proposition}[{\cite[Chapter 8, Lemma 1]{luen}}]\label{lemma: firstorder}
    Let $\msf F$ be a Fr\'{e}chet differentiable convex functional on a real
normed space $\cB$. Let $\cC'$ be a convex cone in $\cB$. A necessary and sufficient condition that $f_0 \in \cP$  minimizes $\msf F$ over $\cC'$ is that
\begin{align*}
    \partial_{f_0}\msf F (f) &\ge 0\qquad \forall\, f \in \cC',\\
    \partial_{f_0}\msf F (f_0) &= 0.
\end{align*}
\end{proposition}
We are interested in the case where the convex cone of interest is the space $\cB$ itself. The lemma above is stated for any real normed space $\cB$. Given that we are interested in Banach spaces, we could state the following more precise statement on the minimum of the functional $\msf F$.
\begin{proposition}[{\cite[Section 7.4, Theorem 1]{luen}}]
Let the real-valued functional \( \msf F \) have a G\^ateaux differential on a vector space \( \cB \). A necessary condition for \( \msf F \) to have an extremum at \( f_0 \in \cB \) is that \( \partial_{f_0} \msf F(h) = 0 \) for all \( h \in \cB \).
\end{proposition}

Now, we state and prove a useful result for proper functionals, \tt{i.e.}
$M: \cB \to \reals$ such that $(\textnormal{dom } \msf F) \neq \emptyset$ and $\msf F(f) \ge - \infty$ for all $f \in \cB$.
%We are interested in functionals $M: \cB \to \reals$ that are \tt{proper}, i.e. $\textnormal{dom } \msf M \neq \empty$ and $\msf M(f) \ge - \infty$ for all $f \in \cB$.

\begin{lemma}\label{lemma: inversemirror}
    Consider a convex, reflexive Banach space $(\cB, \norm{\cdot}_{\cB})$. Let $\msf F: \cB \to \reals$ be a proper, strictly convex and G$\hat{a}$teaux differentiable functional. %Consider $\msf F^*: \cB^* \to \reals$ to be the convex conjugate of $\msf F$. 
    Then, for all $f, f' \in \cB$,
    \begin{align}
        \partial_{f} \msf F = \partial_{f'} \msf F \implies f = f'
    \end{align}
    Furthermore, for any linear functional $\bg{}^* \in \cB^*$, there exists $\hat{f} \in \cB$ such that
    \begin{align*}
        \bg{}^* = \partial_{\hat{f}} \msf F
    \end{align*}
    In order words, the operator $\partial_{(\cdot)} \msf F: \cB \to \cB^*$ is both injective and subjective, where 
    \begin{align*}
        \forall f \in \cB,\,\, f \longmapsto \partial_{(\cdot)} \msf F(f) := \partial_f \msf F \in \cB^*
    \end{align*}
    %\begin{align}
    %  f = \partial_{\bg{}^*} \msf F^*   \label{eq: inverse}
    %\end{align}
%where $\bg{}^* := \partial_f \msf F$. In other words, the Frech$\acute{e}$t derivative of $\msf F$ at $f$ is the inverse of the Frech$\acute{e}$t derivative of the $\msf F^*$ at $\partial_f \msf F$.
\end{lemma}
\begin{proof}
    First, we would show the injectivity of the operator $\partial_{(\cdot)} \msf F$. In order to show that, consider the convex conjugate of $\msf F$, denoted as $\msf F^*$. Note that $\msf F^*: \cB^* \to \reals$,  and  
    \begin{align}
        \forall \bg{}\in\cB^*,\, \msf F^*(\bg{}) := - \inf_{f \in \cB} (-\dist{f}{\bg{}} + \msf F(f)) \label{eq: conjugate}
    \end{align}
    We denote $\hat{\msf F}_{\bg{}}(f) := -\dist{f}{\bg{}} + \msf F(f)$.
    Note that since $\msf F$ is strictly convex, thus $\hat{\msf F}_{\bg{}}$ is strictly convex in $f$. Thus, the objective $\hat{\msf F}_{\bg{}}(f)$ can only have a \tt{unique} minimizer.
    
    Assume that there exists $\hat{f} \in \cB$ such that $\bg{} := \partial_{\hat{f}} \msf F$. Using the first-order optimality condition in \lemref{lemma: firstorder}, $\hat{f}$ is the minimizer of $\hat{\msf F}_{\bg{}}$, but then it is the unique minimizer. This implies that there doesn't exist $f' \neq \hat{f}$ such that $\partial_{f'} \msf F = \partial_{\hat{f}} \msf F$. This completes the proof of the injectivity of the operator $\partial_{(\cdot)} \msf F$.
    
    Now, we would establish the surjectivity of the operator $\partial_{(\cdot)} \msf F$ over $\cB^*$. Using Theorem 2.3.3~\cite{Zlinescu2002ConvexAI}, $\msf F^{**} = \msf F$, i.e.
    \begin{align}
        \forall f' \in \cB,\,\msf F(f') := - \inf_{\hat{\bg{}} \in \cB^*} (-\dist{f'}{\hat{\bg{}}} + \msf F^*(\hat{\bg{}})) \label{eq: dualconjugate}
    \end{align}
    Consider a linear transformation $\bg{}^* \in \cB^*$. Assume that $\hat{\msf F}_{\bg{}^*}$ is minimized at $f_0 \in \cB$. Thus,
    \begin{align}
        \msf F^*(\bg{}^*) = \dist{f_0}{\bg{}^*} - \msf F(f_0) \label{eq: l1}
    \end{align}
    Using \textbf{Young-Fenchel inequality} (Theorem 2.3.1 \cite{Zlinescu2002ConvexAI}), we note that for all $f \in \cB$,
    \begin{align}
        \msf F(f) + \msf F^*(\bg{}^*) \ge \dist{f}{\bg{}^*} \label{eq: l2}
    \end{align}
    Subtracting \eqnref{eq: l1} and \eqnref{eq: l2}, we observe that for all $f \in \cB$,
    \begin{equation*}
        \msf F(f) - \msf F(f_0) \ge \dist{f - f_0}{\bg{}^*}
    \end{equation*}
    This implies that $\bg{}^* \in \partial_{f_0} \msf F$, i.e $\bg{}^*$ is in the subdifferential set of $\partial_{f_0} \msf F$. Since $\msf F$ is G\^{a}teaux differentiable at $f_0$ it must be the case that $\bg{}^* = \partial_{f_0} \msf F$.

    Given that $\bg{}^*$ was picked arbitrarily, we have shown that for any $\bg{}^* \in \cB^*$ there exists $f_0 \in \cB$ such that $\bg{}^* = \partial_{f_0} \msf F$. This completes the proof of the surjectivity of the operator $\partial_{(\cdot)} \msf F$ over $\cB^*$.
    %Now, we would argue that
    %then $\hat{f}$ is the unique minimizer of the objective $(-\dist{f}{\bg{}} + \msf F(f))$. 
    %We define the evaluation of $\msf F^*$ 
\end{proof}

\akash{Is \lemref{lemma: inversemirror} required for main theorem??}


\begin{proposition}[{\cite[Section 7.4, Theorem 2]{luen}}]\label{prop: constfirstorder}
Let \( \msf F \) be a real-valued functional defined on a vector space \( \cB \). Suppose that \( f_0 \) minimizes \( \msf F \) on the convex set \( \Omega \subseteq \cB \) and that \( \msf F \) is G\^ateaux differentiable at \( f_0 \). Then
\[
\partial_{f_0} \msf F(f - f_0) \geq 0
\]
for all \( f \in \Omega \).
\end{proposition}
%Now, we show that the projection operation via $\mf D_\Phi$
One of the most important properties of the projected MDA of \eqnref{eq: constMD} is every gradient step in the dual space $\cB^*$ has a postive component along the direction of the minimizer in the primal space $\cB$. So, the projection operation via $\mf D_\Phi$ retains the essential directions of descent. We formalize this intuition with this result.
%is in the direction of steepest descent (\tt{wrt} to the loss functional) 
\begin{lemma}\label{lemma: natdirection}
 Let $f \in \cB_0 \cap \cC$ and $f' \in \cC$, then
 \begin{align*}
     \inner{\Pi_{\cB_0}^{\Phi}(f') - f,\hspace{1mm} \partial_{\Pi_{\cB_0}^{\Phi}(f')} \Phi - \partial_{f'} \Phi}_{\cB} \le 0
 \end{align*}
    
\end{lemma}
\begin{proof}
    First, note that for any $f' \in \cC$, the map $h\mapsto \mf D_{\Phi}(h,f')$ is convex. Secondly, note that for any $f,f'$ we can write 
    \begin{align}
      \partial_f \mf D_{\Phi}(\cdot,f') = \partial_f \Phi - \partial_{f'} \Phi  \label{eq: proj}
    \end{align}

    %Rest of the proof follows similar steps as provided for Lemma 4.1 (Bubeck's notes) \pp{restate lemma here}.
Note that by definition, $\Pi_{\cB_0}^{\Phi}(f')$ is the minimizer of $\mf D_{\Phi}(f,f')$ in the first component over $\cB_0 \cap \cC$. But using \propref{prop: constfirstorder} 
\begin{align*}
    \inner{f - \Pi_{\cB_0}^{\Phi}(f'),\,\partial_{\Pi_{\cB_0}^{\Phi}(f')} \mf D_{\Phi}(\cdot,f')}_\cB \ge 0, \quad \forall\,f \in \cB_0 \cap \cC
\end{align*}
Now, using the observation in \eqnref{eq: proj}, the main claim of the lemma follows.
\end{proof}

==> sections/notation.tex <==
\section{Notation}

\begin{table}[h]
\begin{center}
% \caption{Notation}
\begin{tabular}{ll}
\toprule
Script & Usage\\
\midrule
     $f,g,h$ &  elements of vector space or dual space\\
     $\x$ & elements of input space\\
     $\alpha,\beta$&
     vectors in euclidean space\\
     $\eta$ & learning rate\\
     $G,H,K$ & bivariate functions such as kernel function and Greens functions\\
     $\mf D$ & Bregman divergence\\
     $\mc H,\mc B, \mc C$& function spaces \\
     $\_^*$ & dual\\
     $\msf A, \msf B,\msf C,\msf L$& nonlinear functionals\\
     $\Phi,\Psi$ & nonlinear functionals\\
     %$\mf A,\mf B,\mf C$ & Space of functions \pp{Don't use}\\
     $\partial_f$ & Fr\'echet derivative, $\partial_f\msf L$ is an element of dual space\\
     $\delta_x$ & evaluation functional  $\delta_x:f\mapsto f(x)$\\
     $\inner{\cdot,\cdot}_{\Banach}$ & $\mc B\times\mc B^*\to\Real$\\
     $\rho, \kappa$ & constants\\
     \bottomrule
\end{tabular}
\end{center}
\end{table}

==> sections/notes.tex <==
\section{Approximate mirror map}

Consider that the \red{dual of the} target classifier has the form $\sum_{i = 1}^n \alpha_ib(x_i,\cdot)$ for scalars $\alpha_i$, in the dual space for given training data $\curlybracket{x_i,y_i}_{i=1}^n$. Now, we note the following dual map for a function $g^* \in L_q$,
\begin{align*}
    g = \frac{(g^*)^{q-1}}{||g^*||_q^{q-2}},
\end{align*}
where $g \in L_p$ and $(p, q)$ is a conjugate pair, i.e. $\frac{1}{p} + \frac{1}{q} = 1$.

Thus, if $f^* := \sum_{i=1}^n \alpha_i \cdot b(x_i,\cdot) \in L_q$, then we could write its dual $L_p$ as 
\begin{align*}
    f = c \paren{\sum_{i=1}^n \alpha_i\cdot b(x_i,\cdot)}^{q-1}
\end{align*}
where $c$ is the solution of the minimization problem
\begin{align*}
    \min{c > 0} \sum_i \paren{c f(x_i) - y_i}^2
\end{align*}
Solving this objective gives us the solution $$c = \frac{\sum_i f(x_i) y_i}{\sum_i f(x_i)^2}$$

\paragraph{Updating the parameters} We denote timed parameters as $\alpha^t$. 


\begin{align*}
    &- 2\eta\sum_{i=1}^n\paren{c f(x_i) - y_i}\cdot G(x_i,\cdot)\\
    =& - 2\eta\sum_{i=1}^n\paren{\paren{\frac{\sum_i f(x_i) y_i}{\sum_i f(x_i)^2}} f(x_i) - y_i}\cdot G(x_i,\cdot)\\
    =& - 2\eta\sum_{i=1}^n\paren{\paren{\frac{\sum_i f(x_i) y_i}{\sum_i f(x_i)^2}} \paren{\sum_{j=1}^n \alpha_j b(x_j,x_i)}^{q-1} - y_i}\cdot G(x_i,\cdot)\\
\end{align*}

Parthe notes 4/5/23: Update equation depends on
\begin{align*}
    (f(X)-Y)_i = f(x_i)-y_i = \round{\sum_{j=1}^n \alpha_i b(x_i, x_j)}^{q-1} - y_i = (B_i\tran\alphavec)^{q-1}-y_i
\end{align*}
\newpage



==> sections/useful_equations.tex <==
Since $p \in (2,\infty)$, note that the map $\Phi_q$ is strongly convex on $\cB^*$, where $\frac{1}{p} + \frac{1}{q} = 1$. Thus, for iterates $g_k$ and $g_{k-1}$ where for any $i$, $g_i$ is the update in the dual space.
Thus, we have :
\begin{align*}
    &\Phi_q(g_k) \ge \Phi_q(g_{k-1}) + (g_k - g_{k-1},\delta_{g_{k-1}} \Phi_q)_{\cB} + \frac{\mu'}{2}||g_k - g_{k-1}||^2_{\cB^*}\\
    &\Phi_q(g_{k-1}) \ge \Phi_q(g_{k}) + (g_{k-1} - g_{k},\delta_{g_{k}} \Phi_q)_{\cB} + \frac{\mu'}{2}||g_k - g_{k-1}||^2_{\cB^*}
\end{align*}
Adding the two we get:
\begin{align*}
    &0 \ge (g_k - g_{k-1}, \delta_{g_{k-1}} \Phi_q - \delta_{g_{k}} \Phi_q)_{\cB} + \frac{\mu'}{2}||g_k - g_{k-1}||^2_{\cB^*}\\
    \implies &0 \ge \eta\cdot(-\mathcal{G}_{f_{k-1}}, f_{k-1} - f_k)_{\cB} + \frac{\mu'\eta^2}{2}\cdot||\mathcal{G}_{f_{k-1}}||^2_{\cB^*}
\end{align*}
Thus, we can write
\begin{align}
    ||f_k - f_{k-1}||_{\cB} \ge \frac{\mu'\eta}{2}\cdot||\mathcal{G}_{f_{k-1}}||_{\cB^*}
\end{align}

\textcolor{red}{For the case when $p \in (1, 2)$, using the strong convexity of squared $\Phi_p$, we have that 
\begin{align*}
    0 &\ge (f_k - f_{k-1}, \delta_{f_{k-1}}\Phi_p - \delta_{f_{k}}\Phi_p )_{\cB} + \mu_p\cdot ||f_k - f_{k-1}||_{\cB}^2\\
    &= (f_k - f_{k-1}, g_{k-1} - g_k)_{\cB} + \mu_p\cdot ||f_k - f_{k-1}||_{\cB}^2\\
    &= \eta\cdot (f_k - f_{k-1}, \mathcal{G}_{f_{k-1}})_{\cB} + \mu_p\cdot ||f_k - f_{k-1}||_{\cB}^2
\end{align*}
}

Using the strong convexity of $\mathcal{L}$, we get that
\begin{align*}
    0 \ge (f_k - f_{k-1}, \delta_{f_{k-1}} \mathcal{L})_{\cB^*} + \frac{\mu}{2}||f_k - f_{k-1}||_{\cB}^2 = (f_k - f_{k-1}, \mathcal{G}_{f_{k-1}})_{\cB^*} + \frac{\mu}{2}||f_k - f_{k-1}||_{\cB}^2
\end{align*}
where we used the inequality that $\mathcal{L}(f_{k-1}) \ge  \mathcal{L}(f_{k})$.

Now, using $L$-Lipsitz property of $\mathcal{L}$ we note that  
\begin{align*}
    \mathcal{L}(f_k) &\le \mathcal{L}(f_{k-1}) + (f_k - f_{k-1}, \mathcal{G}_{f_{k-1}})_{\cB^*} + \frac{L}{2}||f_k - f_{k-1}||_{\cB}^2\\
    &\le \mathcal{L}(f_{k-1}) + \paren{\frac{L}{2} - \frac{\mu}{2}}\cdot||f_k - f_{k-1}||_{\cB}^2\\
    &\le \mathcal{L}(f_{k-1}) - \paren{\frac{\mu}{2} - \frac{L}{2}}\cdot \frac{2}{\mu'\eta} \cdot ||\mathcal{G}_{f_{k-1}}||^2_{\cB^*}\\
    &\le \mathcal{L}(f_{k-1}) - \frac{(\mu - L)}{\mu'\eta} \cdot ||\mathcal{G}_{f_{k-1}}||^2_{\cB^*}
\end{align*}


Now, we note that 
\begin{align*}
    \mathcal{L}(f^*) &:= \inf_{f \in \cB} \mathcal{L}(f)\\
    & = \inf_{f \in \cB} \mathcal{L}(f_k + f)\\
    & \ge \inf_{f \in \cB} \mathcal{L}(f_k) + (f, \delta_{f_k} \mathcal{L})_{\cB^*} + \frac{\mu}{2}\cdot||f||_{\cB}\\
    & = \mathcal{L}(f_k) - \frac{1}{2\mu}\cdot ||\mathcal{G}_{f_k}||_{\cB^*}
\end{align*}
\begin{align*}
    \mathcal{L}(f_k) &\le \mathcal{L}(f_{k-1}) - \frac{\mu - L}{\mu'\eta}\cdot||\mathcal{G}_{f_{k-1}}||_{\cB^*}\\
    &\le \mathcal{L}(f_{k-1}) + \frac{2\mu(\mu - L)}{\mu'\eta}\cdot(\mathcal{L}(f^*) - \mathcal{L}(f_{k-1})) \\
  \mathcal{L}(f_k) - \mathcal{L}(f^*)  &\le -(\mathcal{L}(f^*) - \mathcal{L}(f_{k-1})) + \frac{2\mu(\mu - L)}{\mu'\eta}\cdot(\mathcal{L}(f^*) - \mathcal{L}(f_{k-1}))\\
  &\le \paren{1 - \frac{2\mu(\mu - L)}{\mu'\eta}}(\mathcal{L}(f_{k-1}) - \mathcal{L}(f^*))\\
  &\vdots\\
  &\vdots\\
  &= \paren{1 - \frac{2\mu(\mu - L)}{\mu'\eta}}^{k}(\mathcal{L}(f_{0}) - \mathcal{L}(f^*))\\
  &\le C\cdot e^{-k\cdot\frac{2\mu(\mu - L)}{\mu'\eta}}
\end{align*}
